High precision radial velocities with GIANO spectra

Radial velocities (RV) measured from near-infrared (NIR) spectra are a potentially excellent tool to search for extrasolar planets around cool or active stars. High resolution infrared (IR) spectrographs now available are reaching the high precision of visible instruments, with a constant improvement over time. GIANO is an infrared echelle spectrograph at the Telescopio Nazionale Galileo (TNG) and it is a powerful tool to provide high resolution spectra for accurate RV measurements of exoplanets and for chemical and dynamical studies of stellar or extragalactic objects. No other high spectral resolution IR instrument has GIANO's capability to cover the entire NIR wavelength range (0.95-2.45 micron) in a single exposure. In this paper we describe the ensemble of procedures that we have developed to measure high precision RVs on GIANO spectra acquired during the Science Verification (SV) run, using the telluric lines as wavelength reference. We used the Cross Correlation Function (CCF) method to determine the velocity for both the star and the telluric lines. For this purpose, we constructed two suitable digital masks that include about 2000 stellar lines, and a similar number of telluric lines. The method is applied to various targets with different spectral type, from K2V to M8 stars. We reached different precisions mainly depending on the H -magnitudes: for H ~ 5 we obtain an rms scatter of ~ 10 m s-1, while for H ~ 9 the standard deviation increases to ~ 50 - 80 m s-1. The corresponding theoretical error expectations are ~4 m s-1 and 30 m s-1, respectively. Finally we provide the RVs measured with our procedure for the targets observed during GIANO Science Verification.

==> biblio3.tex <==
\bibitem[{{Bailey} et~al(2012){Bailey}, {White}, {Blake}, {Charbonneau},
  {Barman}, {Tanner}, and {Torres}}]{2012ApJ...749...16B}
{Bailey} JI III, {White} RJ, {Blake} CH, {Charbonneau} D, {Barman} TS, {Tanner}
  AM, {Torres} G (2012) {Precise Infrared Radial Velocities from Keck/NIRSPEC
  and the Search for Young Planets}. ApJ 749:16,
  %\doi{10.1088/0004-637X/749/1/16}, %\eprint{1202.0300}

\bibitem[{{Baranne} et~al(1979){Baranne}, {Mayor}, and
  {Poncet}}]{1979VA.....23..279B}
{Baranne} A, {Mayor} M, {Poncet} JL (1979) {CORAVEL - A new tool for radial
  velocity measurements}. Vistas in Astronomy 23:279--316,
  %\doi{10.1016/0083-6656(79)90016-3}

\bibitem[{{Batten}(1983)}]{1983BICDS..24....3B}
{Batten} AH (1983) {Standard Velocity Stars}. Bulletin d'Information du Centre
  de Donnees Stellaires 24:3

\bibitem[{{Bean} et~al(2010{\natexlab{a}}){Bean}, {Seifahrt}, {Hartman},
  {Nilsson}, {Reiners}, {Dreizler}, {Henry}, and
  {Wiedemann}}]{2010ApJ...711L..19B}
{Bean} JL, {Seifahrt} A, {Hartman} H, {Nilsson} H, {Reiners} A, {Dreizler} S,
  {Henry} TJ, {Wiedemann} G (2010{\natexlab{a}}) {The Proposed Giant Planet
  Orbiting VB 10 Does Not Exist}. ApJl 711:L19--L23,
  %\doi{10.1088/2041-8205/711/1/L19}

\bibitem[{{Bean} et~al(2010{\natexlab{b}}){Bean}, {Seifahrt}, {Hartman},
  {Nilsson}, {Wiedemann}, {Reiners}, {Dreizler}, and
  {Henry}}]{2010ApJ...713..410B}
{Bean} JL, {Seifahrt} A, {Hartman} H, {Nilsson} H, {Wiedemann} G, {Reiners} A,
  {Dreizler} S, {Henry} TJ (2010{\natexlab{b}}) {The CRIRES Search for Planets
  Around the Lowest-mass Stars. I. High-precision Near-infrared Radial
  Velocities with an Ammonia Gas Cell}. ApJ 713:410--422,
  %\doi{10.1088/0004-637X/713/1/410}, %\eprint{0911.3148}

\bibitem[{{Berta} et~al(2011){Berta}, {Charbonneau}, {Bean}, {Irwin}, {Burke},
  {D{\'e}sert}, {Nutzman}, and {Falco}}]{2011ApJ...736...12B}
{Berta} ZK, {Charbonneau} D, {Bean} J, {Irwin} J, {Burke} CJ, {D{\'e}sert} JM,
  {Nutzman} P, {Falco} EE (2011) {The GJ1214 Super-Earth System: Stellar
  Variability, New Transits, and a Search for Additional Planets}. ApJ 736:12,
  %\doi{10.1088/0004-637X/736/1/12}, %\eprint{1012.0518}

\bibitem[{{Blake} et~al(2010){Blake}, {Charbonneau}, and
  {White}}]{2010ApJ...723..684B}
{Blake} CH, {Charbonneau} D, {White} RJ (2010) {The NIRSPEC Ultracool Dwarf
  Radial Velocity Survey}. ApJ 723:684--706, %\doi{10.1088/0004-637X/723/1/684},
  %\eprint{1008.3874}

\bibitem[{{Charbonneau} et~al(2009){Charbonneau}, {Berta}, {Irwin}, {Burke},
  {Nutzman}, {Buchhave}, {Lovis}, {Bonfils}, {Latham}, {Udry}, {Murray-Clay},
  {Holman}, {Falco}, {Winn}, {Queloz}, {Pepe}, {Mayor}, {Delfosse}, and
  {Forveille}}]{2009Natur.462..891C}
{Charbonneau} D, {Berta} ZK, {Irwin} J, {Burke} CJ, {Nutzman} P, {Buchhave} LA,
  {Lovis} C, {Bonfils} X, {Latham} DW, {Udry} S, {Murray-Clay} RA, {Holman} MJ,
  {Falco} EE, {Winn} JN, {Queloz} D, {Pepe} F, {Mayor} M, {Delfosse} X,
  {Forveille} T (2009) {A super-Earth transiting a nearby low-mass star}. \nat
  462:891--894, %\doi{10.1038/nature08679}, %\eprint{0912.3229}

\bibitem[{{Crifo} et~al(2010){Crifo}, {Jasniewicz}, {Soubiran}, {Katz},
  {Siebert}, {Veltz}, and {Udry}}]{2010A&A...524A..10C}
{Crifo} F, {Jasniewicz} G, {Soubiran} C, {Katz} D, {Siebert} A, {Veltz} L,
  {Udry} S (2010) {Towards a new full-sky list of radial velocity standard
  stars}. \aap 524:A10, %\doi{10.1051/0004-6361/201015315}, %\eprint{1010.0613}

\bibitem[{{Cutri} et~al(2003){Cutri}, {Skrutskie}, {van Dyk}, {Beichman},
  {Carpenter}, {Chester}, {Cambresy}, {Evans}, {Fowler}, {Gizis}, {Howard},
  {Huchra}, {Jarrett}, {Kopan}, {Kirkpatrick}, {Light}, {Marsh}, {McCallon},
  {Schneider}, {Stiening}, {Sykes}, {Weinberg}, {Wheaton}, {Wheelock}, and
  {Zacarias}}]{2003yCat.2246....0C}
{Cutri} RM, {Skrutskie} MF, {van Dyk} S, {Beichman} CA, {Carpenter} JM,
  {Chester} T, {Cambresy} L, {Evans} T, {Fowler} J, {Gizis} J, {Howard} E,
  {Huchra} J, {Jarrett} T, {Kopan} EL, {Kirkpatrick} JD, {Light} RM, {Marsh}
  KA, {McCallon} H, {Schneider} S, {Stiening} R, {Sykes} M, {Weinberg} M,
  {Wheaton} WA, {Wheelock} S, {Zacarias} N (2003) {VizieR Online Data Catalog:
  2MASS All-Sky Catalog of Point Sources (Cutri+ 2003)}. VizieR Online Data
  Catalog 2246

\bibitem[{{Figueira} et~al(2010{\natexlab{a}}){Figueira}, {Pepe}, {Lovis}, and
  {Mayor}}]{2010A&A...515A.106F}
{Figueira} P, {Pepe} F, {Lovis} C, {Mayor} M (2010{\natexlab{a}}) {Evaluating
  the stability of atmospheric lines with HARPS}. \aap 515:A106,
  %\doi{10.1051/0004-6361/201014005}, %\eprint{1003.0541}

\bibitem[{{Figueira} et~al(2010{\natexlab{b}}){Figueira}, {Pepe}, {Melo},
  {Santos}, {Lovis}, {Mayor}, {Queloz}, {Smette}, and
  {Udry}}]{2010A&A...511A..55F}
{Figueira} P, {Pepe} F, {Melo} CHF, {Santos} NC, {Lovis} C, {Mayor} M, {Queloz}
  D, {Smette} A, {Udry} S (2010{\natexlab{b}}) {Radial velocities with CRIRES.
  Pushing precision down to 5-10 m/s}. \aap 511:A55,
  %\doi{10.1051/0004-6361/200912681}, %\eprint{0912.2643}

\bibitem[{{Goldberg} and {M{\"u}ller}(1953)}]{1953ApJ...118..397G}
{Goldberg} L, {M{\"u}ller} EA (1953) {Carbon Monoxide in the Sun.} ApJ 118:397,
  %\doi{10.1086/145768}

\bibitem[{{Henry} et~al(2006){Henry}, {Koerner}, {Jao}, {Subasavage}, {Ianna},
  and {RECONS}}]{2006AAS...209.2404H}
{Henry} TJ, {Koerner} DW, {Jao} WC, {Subasavage} JP, {Ianna} PA, {RECONS}
  (2006) {Clandestine Companions of Nearby Red Dwarfs}. In: American
  Astronomical Society Meeting Abstracts, Bulletin of the American Astronomical
  Society, vol~38, p 933

\bibitem[{{Howard} et~al(2014){Howard}, {Marcy}, {Fischer}, {Isaacson},
  {Muirhead}, {Henry}, {Boyajian}, {von Braun}, {Becker}, {Wright}, and
  {Johnson}}]{2014ApJ...794...51H}
{Howard} AW, {Marcy} GW, {Fischer} DA, {Isaacson} H, {Muirhead} PS, {Henry} GW,
  {Boyajian} TS, {von Braun} K, {Becker} JC, {Wright} JT, {Johnson} JA (2014)
  {The NASA-UC-UH ETA-Earth Program. IV. A Low-mass Planet Orbiting an M Dwarf
  3.6 PC from Earth}. ApJ 794:51, %\doi{10.1088/0004-637X/794/1/51},
  %\eprint{1408.5645}

\bibitem[{{Hu{\'e}lamo} et~al(2008){Hu{\'e}lamo}, {Figueira}, {Bonfils},
  {Santos}, {Pepe}, {Gillon}, {Azevedo}, {Barman}, {Fern{\'a}ndez}, {di Folco},
  {Guenther}, {Lovis}, {Melo}, {Queloz}, and {Udry}}]{2008A&A...489L...9H}
{Hu{\'e}lamo} N, {Figueira} P, {Bonfils} X, {Santos} NC, {Pepe} F, {Gillon} M,
  {Azevedo} R, {Barman} T, {Fern{\'a}ndez} M, {di Folco} E, {Guenther} EW,
  {Lovis} C, {Melo} CHF, {Queloz} D, {Udry} S (2008) {TW Hydrae: evidence of
  stellar spots instead of a Hot Jupiter}. \aap 489:L9--L13,
  %\doi{10.1051/0004-6361:200810596}, %\eprint{0808.2386}

\bibitem[{{Isaacson} and {Fischer}(2010)}]{2010ApJ...725..875I}
{Isaacson} H, {Fischer} D (2010) {Chromospheric Activity and Jitter
  Measurements for 2630 Stars on the California Planet Search}. ApJ
  725:875--885, %\doi{10.1088/0004-637X/725/1/875}, %\eprint{1009.2301}

\bibitem[{{Kaltenegger} and {Traub}(2009)}]{2009ApJ...698..519K}
{Kaltenegger} L, {Traub} WA (2009) {Transits of Earth-like Planets}. ApJ
  698:519--527, %\doi{10.1088/0004-637X/698/1/519}, %\eprint{0903.3371}

\bibitem[{{Kasting} et~al(1993){Kasting}, {Whitmire}, and
  {Reynolds}}]{1993Icar..101..108K}
{Kasting} JF, {Whitmire} DP, {Reynolds} RT (1993) {Habitable Zones around Main
  Sequence Stars}. \icarus 101:108--128, %\doi{10.1006/icar.1993.1010}

\bibitem[{{L{\'e}pine} and {Gaidos}(2011)}]{2011AJ....142..138L}
{L{\'e}pine} S, {Gaidos} E (2011) {An All-sky Catalog of Bright M Dwarfs}. \aj
  142:138, %\doi{10.1088/0004-6256/142/4/138}, %\eprint{1108.2719}

\bibitem[{{Lovis} et~al(2006){Lovis}, {Mayor}, {Pepe}, {Alibert}, {Benz},
  {Bouchy}, {Correia}, {Laskar}, {Mordasini}, {Queloz}, {Santos}, {Udry},
  {Bertaux}, and {Sivan}}]{2006Natur.441..305L}
{Lovis} C, {Mayor} M, {Pepe} F, {Alibert} Y, {Benz} W, {Bouchy} F, {Correia}
  ACM, {Laskar} J, {Mordasini} C, {Queloz} D, {Santos} NC, {Udry} S, {Bertaux}
  JL, {Sivan} JP (2006) {An extrasolar planetary system with three Neptune-mass
  planets}. \nat 441:305--309, %\doi{10.1038/nature04828},
  %\eprint{astro-ph/0703024}

\bibitem[{{Mart{\'{\i}}nez-Arn{\'a}iz} et~al(2010){Mart{\'{\i}}nez-Arn{\'a}iz},
  {Maldonado}, {Montes}, {Eiroa}, and {Montesinos}}]{2010A&A...520A..79M}
{Mart{\'{\i}}nez-Arn{\'a}iz} R, {Maldonado} J, {Montes} D, {Eiroa} C,
  {Montesinos} B (2010) {Chromospheric activity and rotation of FGK stars in
  the solar vicinity. An estimation of the radial velocity jitter}. \aap
  520:A79, %\doi{10.1051/0004-6361/200913725}, %\eprint{1002.4391}

\bibitem[{{Mayor} et~al(1995){Mayor}, {Queloz}, {Marcy}, {Butler}, {Noyes},
  {Korzennik}, {Krockenberger}, {Nisenson}, {Brown}, {Kennelly}, {Rowland},
  {Horner}, {Burki}, {Burnet}, and {Kunzli}}]{1995IAUC.6251....1M}
{Mayor} M, {Queloz} D, {Marcy} G, {Butler} P, {Noyes} R, {Korzennik} S,
  {Krockenberger} M, {Nisenson} P, {Brown} T, {Kennelly} T, {Rowland} C,
  {Horner} S, {Burki} G, {Burnet} M, {Kunzli} M (1995) {51 Pegasi}. \iaucirc
  6251

\bibitem[{{Mishenina} et~al(2004){Mishenina}, {Soubiran}, {Kovtyukh}, and
  {Korotin}}]{2004A&A...418..551M}
{Mishenina} TV, {Soubiran} C, {Kovtyukh} VV, {Korotin} SA (2004) {On the
  correlation of elemental abundances with kinematics among galactic disk
  stars}. \aap 418:551--562, %\doi{10.1051/0004-6361:20034454},
  %\eprint{astro-ph/0401234}

\bibitem[{{Mohanty} and {Basri}(2003)}]{2003ApJ...583..451M}
{Mohanty} S, {Basri} G (2003) {Rotation and Activity in Mid-M to L Field
  Dwarfs}. ApJ 583:451--472, %\doi{10.1086/345097}, %\eprint{astro-ph/0201455}

\bibitem[{{Mohler} et~al(1953){Mohler}, {Pierce}, {McMath}, and
  {Goldberg}}]{1953ApJ...117...41M}
{Mohler} OC, {Pierce} AK, {McMath} RR, {Goldberg} L (1953) {Table of Infrared
  Solar Lines, 1.4-2.5 {$\mu$}.} ApJ 117:41, %\doi{10.1086/145667}

\bibitem[{{Oliva} et~al(2006){Oliva}, {Origlia}, {Baffa}, {Biliotti}, {Bruno},
  {D'Amato}, {Del Vecchio}, {Falcini}, {Gennari}, {Ghinassi}, {Giani},
  {Gonzalez}, {Leone}, {Lolli}, {Lodi}, {Maiolino}, {Mannucci}, {Marcucci},
  {Mochi}, {Montegriffo}, {Rossetti}, {Scuderi}, and
  {Sozzi}}]{2006SPIE.6269E..19O}
{Oliva} E, {Origlia} L, {Baffa} C, {Biliotti} C, {Bruno} P, {D'Amato} F, {Del
  Vecchio} C, {Falcini} G, {Gennari} S, {Ghinassi} F, {Giani} E, {Gonzalez} M,
  {Leone} F, {Lolli} M, {Lodi} M, {Maiolino} R, {Mannucci} F, {Marcucci} G,
  {Mochi} I, {Montegriffo} P, {Rossetti} E, {Scuderi} S, {Sozzi} M (2006) {The
  GIANO-TNG spectrometer}. In: Society of Photo-Optical Instrumentation
  Engineers (SPIE) Conference Series, \procspie, vol 6269, p 626919,
  %\doi{10.1117/12.670006}

\bibitem[{{Oliva} et~al(2012){Oliva}, {Origlia}, {Maiolino}, {Baffa},
  {Biliotti}, {Bruno}, {Falcini}, {Gavriousev}, {Ghinassi}, {Giani},
  {Gonzalez}, {Leone}, {Lodi}, {Massi}, {Mochi}, {Montegriffo}, {Pedani},
  {Rossetti}, {Scuderi}, {Sozzi}, and {Tozzi}}]{2012SPIE.8446E..3TO}
{Oliva} E, {Origlia} L, {Maiolino} R, {Baffa} C, {Biliotti} V, {Bruno} P,
  {Falcini} G, {Gavriousev} V, {Ghinassi} F, {Giani} E, {Gonzalez} M, {Leone}
  F, {Lodi} M, {Massi} F, {Mochi} I, {Montegriffo} P, {Pedani} M, {Rossetti} E,
  {Scuderi} S, {Sozzi} M, {Tozzi} A (2012) {The GIANO spectrometer: towards its
  first light at the TNG}. In: Ground-based and Airborne Instrumentation for
  Astronomy IV, \procspie, vol 8446, p 84463T, %\doi{10.1117/12.925274}

\bibitem[{{Origlia} et~al(2014){Origlia}, {Oliva}, {Baffa}, {Falcini}, {Giani},
  {Massi}, {Montegriffo}, {Sanna}, {Scuderi}, {Sozzi}, {Tozzi}, {Carleo},
  {Gratton}, {Ghinassi}, and {Lodi}}]{2014SPIE.9147E..1EO}
{Origlia} L, {Oliva} E, {Baffa} C, {Falcini} G, {Giani} E, {Massi} F,
  {Montegriffo} P, {Sanna} N, {Scuderi} S, {Sozzi} M, {Tozzi} A, {Carleo} I,
  {Gratton} R, {Ghinassi} F, {Lodi} M (2014) {High resolution near IR
  spectroscopy with GIANO-TNG}. In: Ground-based and Airborne Instrumentation
  for Astronomy V, \procspie, vol 9147, p 91471E, %\doi{10.1117/12.2054743}

\bibitem[{{Pepe} et~al(2004){Pepe}, {Mayor}, {Queloz}, {Benz}, {Bonfils},
  {Bouchy}, {Lo Curto}, {Lovis}, {M{\'e}gevand}, {Moutou}, {Naef}, {Rupprecht},
  {Santos}, {Sivan}, {Sosnowska}, and {Udry}}]{2004A&A...423..385P}
{Pepe} F, {Mayor} M, {Queloz} D, {Benz} W, {Bonfils} X, {Bouchy} F, {Lo Curto}
  G, {Lovis} C, {M{\'e}gevand} D, {Moutou} C, {Naef} D, {Rupprecht} G, {Santos}
  NC, {Sivan} JP, {Sosnowska} D, {Udry} S (2004) {The HARPS search for southern
  extra-solar planets. I. HD 330075 b: A new ``hot Jupiter''}. \aap
  423:385--389, %\doi{10.1051/0004-6361:20040389}, %\eprint{astro-ph/0405252}

\bibitem[{{Pravdo} and {Shaklan}(2009)}]{2009ApJ...700..623P}
{Pravdo} SH, {Shaklan} SB (2009) {An ultracool Star's Candidate Planet}. ApJ
  700:623--632, %\doi{10.1088/0004-637X/700/1/623}, %\eprint{0906.0544}

\bibitem[{{Queloz} et~al(2001){Queloz}, {Henry}, {Sivan}, {Baliunas}, {Beuzit},
  {Donahue}, {Mayor}, {Naef}, {Perrier}, and {Udry}}]{2001A&A...379..279Q}
{Queloz} D, {Henry} GW, {Sivan} JP, {Baliunas} SL, {Beuzit} JL, {Donahue} RA,
  {Mayor} M, {Naef} D, {Perrier} C, {Udry} S (2001) {No planet for HD 166435}.
  \aap 379:279--287, %\doi{10.1051/0004-6361:20011308},
  %\eprint{astro-ph/0109491}

\bibitem[{{Rodler} et~al(2012){Rodler}, {Deshpande}, {Zapatero Osorio},
  {Mart{\'{\i}}n}, {Montgomery}, {Del Burgo}, and
  {Creevey}}]{2012A&A...538A.141R}
{Rodler} F, {Deshpande} R, {Zapatero Osorio} MR, {Mart{\'{\i}}n} EL,
  {Montgomery} MM, {Del Burgo} C, {Creevey} OL (2012) {Search for radial
  velocity variations in eight M-dwarfs with NIRSPEC/Keck II}. \aap 538:A141,
  %\doi{10.1051/0004-6361/201117577}, %\eprint{1112.1382}

\bibitem[{{Seifahrt} and {K{\"a}ufl}(2008)}]{2008A&A...491..929S}
{Seifahrt} A, {K{\"a}ufl} HU (2008) {High precision radial velocity
  measurements in the infrared. A first assessment of the RV stability of
  CRIRES}. \aap 491:929--939, %\doi{10.1051/0004-6361:200810174},
  %\eprint{0809.1435}

\bibitem[{{Setiawan} et~al(2008){Setiawan}, {Henning}, {Launhardt},
  {M{\"u}ller}, {Weise}, and {K{\"u}rster}}]{2008Natur.451...38S}
{Setiawan} J, {Henning} T, {Launhardt} R, {M{\"u}ller} A, {Weise} P,
  {K{\"u}rster} M (2008) {A young massive planet in a star-disk system}. \nat
  451:38--41, %\doi{10.1038/nature06426}

\bibitem[{{Strassmeier} et~al(2000){Strassmeier}, {Washuettl}, {Granzer},
  {Scheck}, and {Weber}}]{2000A&AS..142..275S}
{Strassmeier} K, {Washuettl} A, {Granzer} T, {Scheck} M, {Weber} M (2000) {The
  Vienna-KPNO search for Doppler-imaging candidate stars. I. A catalog of
  stellar-activity indicators for 1058 late-type Hipparcos stars}. \aaps
  142:275--311, %\doi{10.1051/aas:2000328}

\bibitem[{{Tozzi} et~al(2014){Tozzi}, {Oliva}, {Origlia}, {Baffa}, {Biliotti},
  {Falcini}, {Giani}, {Iuzzolino}, {Massi}, {Sanna}, {Scuderi}, and
  {Sozzi}}]{2014SPIE.9147E..9NT}
{Tozzi} A, {Oliva} E, {Origlia} L, {Baffa} C, {Biliotti} V, {Falcini} G,
  {Giani} E, {Iuzzolino} M, {Massi} F, {Sanna} N, {Scuderi} S, {Sozzi} M (2014)
  {The fiber-fed preslit of GIANO at T.N.G.} In: Ground-based and Airborne
  Instrumentation for Astronomy V, \procspie, vol 9147, p 91479N,
  %\doi{10.1117/12.2054094}, %\eprint{1407.3126}
